Completions and Terminal Monads

We consider the terminal monad among those preserving the objects of a subcategory, and in particular preserving the image of a monad. Several common monads are shown to be uniquely characterized by the property of being terminal objects in the category of co-augmented endo-functors. Once extended to infinity categories, this gives, for example, a complete characterization of the well-known Bousfield-Kan R-homology completion. In addition, we note that an idempotent pro-completion tower can be associated with any co-augmented endo functor M, whose limit is the terminal monad that preserves the closure of ImM, the image of M, under finite limits. We conclude that some basic properties of the homological completion tower of a space can be formulated and proved for general monads over any category with limits, and characterized as universal

==> remarkonmonads.tex <==
there is an interesting phenomena re
the structured double dual:

as Sergei noticed $T_3$ is equal to $U,$ the ultrafilter functor. But $U$ can also be written as
the double dual $DD^\infty_3$ namely using the full
operad $O_3.$

so it seems that there is some sort of  equivalence between the double duals

$$ DD^{End 3}(3)= DD^1_3\cong  DD^\infty_3$$

Namely, as a functor on Sets the double dual stabilizes at $r-ity =1,$ for the object 3.

Now fin the category of vector spaces the double dual stabilizes at r-ity=0 since one need not use
the endomorphism in the dual but uses only naive double dual.

So it seems that the reason might be that the 
{\em lower r-ity operads determine the higher ones.} Namely, every operation

$V\times V\to V$ can be reduced to lineal maps of 
vector spaces.

In Sets, for the set $A=3$ the double dual with respect to the operad $O_3$ stabilizes at r-ity one.
but not every two places operation on 3 can be expressed
in terms of one place operation i.e. in terms of a combination of endo-morphism. So it seems that there are more  information in two places operation than in any combination of endo-morphisms. 

So how exactly the functor $DD_i_3$ stabilizes??
--------------------------


In general, what is the relation between the $r-ity$ filtration of the double dual and the co-simplicial filtration..?? is the $DD_O$ for an object  equivalent to the total space for the naive double dual?
---------------------------------

Questions: Feb 11 2023

in the category of groups we know that localization of abelian group is abelian.
(no such thm for nilpotent gps--it is a conjecture)

Now question: Let G be a group and A abelian group.  Is it true that 

T_G(A) is abelian??

same for nilpotent groups T_G(Nil)=nil??

Consider the map $Z\to T_G(Z)$ 
We get a map oof Z namely an elemnt in the unknown group $T_G(Z).$

this unknown group  is some version of G itself being the end(G)-equivarint maps 

|G|---->G.

so $T_G(Z)$ looks like $G^{G/End G}$  ie some power
of G up to an isomorphism.. but what kind of group has a canonical element ie a map from Z to it??
it seems that 1 in Z maps to a diagonal element $(g_1,g_2,g_3,....g_l)$ when these $g_i$ represent the endomorphism-classes of |G| the underlying set of G. But waht is the corresponing idempotent $L_G$ and how the kir tower looks for this monad $T_G??$


------------------------------------------

question: Feb 11 2023

there is no natural perfect quotient of a group! there is no natural nilpotent subgroup
of a group!!

Notice that there is a natural nilpotent 
covering space of a connected space!..
but no natural (non-trivial) FX-->X
where FX is a GEM..or a truncated nilpotent space. (i.e. truly nilpotent)

similarly, there is no natural finite quotient 
of a group! or p-torsion quotient ..

but there is a nonzero divisible "quotient"

Conj: Let Var be a variety of groups.

If there is a non-zero co-augmented functor
Gps--->Var  (G--->V(G)
Then there is NO augmented functor

Gps --->Var  (V(G)----->G)

so since there are nilpotent quotients there are no nilpotent subgroups since there is a perfect subgroup there is no perfect quotient.

there is a uniquely divisible "quotient" i.e.no trivial aug  ==> there is no uniquely divisible 
subgroup..

There is a profinite quotient .. ===> exists  NO profinite "subgroup" etc.


since there is a free augmented .. there is no free co-augmented.


same for spaces!


for some varieties such as finite groups, there is neither quotient nor subgroups!!


Moreover, the only functors from
Grps---->finitegrps are constant functors:

Fun (Grps, FinGrps)= finGroups.

Fun (Spaces, 1-dim spaces)=1-dim spaces

Fun (Sets, limited-cardinalSets)=limited-cardinalSets



------------------------------------------

Question: consider T in the category of groups.

Let G be a group and A an abelian group.

Is it true that $T_G(A)$ is abelian?

Does $T_G$ preserve the finiteness of a group?

Notice that for set the answer is yes! since if G above is infinite then since $T_G$ preserves G it preserves any retract of G, in particular any finite set. Same for other varieties e.g. uniquely divisible. 

Note that $T_G$ does not respect finite products.
------------------------------

Is it true if H is the direct product of 
all finite groups (ALL!) then $T_H$ is the 
profinite completion? It preserves all finite groups, and the product is pro-finite, being the inverse limit of a system of finite groups; it maps
to the profinite completion

$$T_H\to Pro$$

since the latter is the terminal that preserves every finite group. But it seems that the profinite completion of the product
is equal to the product so the profinite completion must map back to $T_H.$

Guess: $$ T_H\cong Pro $$
